Semi-Supervised Few-Shot Learning with Prototypical Random Walks

Recent progress has shown that few-shot learning can be improved with access to unlabelled data, known as semi-supervised few-shot learning(SS-FSL). We introduce an SS-FSL approach, dubbed as Prototypical Random Walk Networks(PRWN), built on top of Prototypical Networks (PN). We develop a random walk semi-supervised loss that enables the network to learn representations that are compact and well-separated. Our work is related to the very recent development of graph-based approaches for few-shot learning. However, we show that compact and well-separated class representations can be achieved by modeling our prototypical random walk notion without needing additional graph-NN parameters or requiring a transductive setting where a collective test set is provided. Our model outperforms baselines in most benchmarks with significant improvements in some cases. Our model, trained with 40$\%$ of the data as labeled, compares competitively against fully supervised prototypical networks, trained on 100$\%$ of the labels, even outperforming it in the 1-shot mini-Imagenet case with 50.89$\%$ to 49.4$\%$ accuracy. We also show that our loss is resistant to distractors, unlabeled data that does not belong to any of the training classes, and hence reflecting robustness to labeled/unlabeled class distribution mismatch. Associated GitHub page can be found at https://prototypical-random-walk.github.io.

==> table1.tex <==
\pdfoutput=1
\begin{table*}[t!]
\centering
    \caption{Semi-Supervised Meta-Learning + Ablation Study} \label{tbl_SOA}
\resizebox{0.98\textwidth}{!}{
    \begin{tabular}{l c c c c c} 
     \toprule
     \multirow{2}{*}{Model}     & Omniglot &        \multicolumn{2}{ c }{Mini-Imagenet}  &  \multicolumn{2}{ c }{Tiered-Imagenet}\\ 
                                &  1-shot  &                 1-shot & 5-shot &                 1-shot & 5-shot\\
     \toprule
    PN$_{all}$\citep{snell2017prototypical}& 98.8                  & 49.4                  & 68.2 & 53.6 & 74.34\\
    \midrule
%    PN~\citep{ren2018metalearning}   & 94.62 $\pm$ 0.09        & 43.61 $\pm$ 0.27        & 59.08 $\pm$ 0.22 \\
%    GNN-LabeledOnly~\citep{garcia2017few} &  N/A &  N/A & 56.91 $\pm$ N/A\\
%    EGNN-LabeledOnly~\citep{kim2019edge} &  N/A &  N/A & N/A\\
    PN~\citep{ren2018metalearning}   & 94.62 $\pm$ 0.09        & 43.61 $\pm$ 0.27        & 59.08 $\pm$ 0.22 &46.52$ \pm $ 0.52    & 66.15$ \pm $ 0.22\\
     \midrule    
    MetaGAN~\citep{zhang2018metagan}                          & 97.58 $\pm$ 0.07        & 50.35 $\pm$ 0.23        & 64.43 $\pm$ 0.27 & N/A & N/A\\
%    GNN-Semi~\citep{garcia2017few} &  N/A &  N/A & 58.76 $\pm$ N/A\\
    EGNN-Semi~\citep{kim2019edge} &  N/A &  N/A & 62.52  $\pm$ N/A  & N/A & \textbf{70.98} $\pm$ N/A \\
%    PRWN (Ours)                      & \textbf{98.28} $\pm$ \textbf{0.15}     & \textbf{50.89} $\pm$ \textbf{0.22}   & \textbf{67.82} $\pm$ \textbf{0.19}\\
    PN$_{VAT}$ (Ours)                     &  97.14 $\pm$ 0.16        & 49.18 $\pm$ 0.22            & 66.94 $\pm$ 0.20 & N/A & N/A\\ 
    PRWN (Ours)                      & \textbf{98.28} $\pm$ \textbf{0.15}     & \textbf{50.89} $\pm$ \textbf{0.22}   & \textbf{67.82} $\pm$ \textbf{0.19} & \textbf{54.87} $\pm$ \textbf{0.46}  & 70.52 $\pm$ 0.43\\
     \midrule
    PN + Semi-supervised inference\citep{ren2018metalearning}     & 97.45 $\pm$ 0.05  & 49.98 $\pm$ 0.34   & 63.77 $\pm$ 0.20 & 50.74 $\pm$ 0.75   & 69.37 $\pm$ 0.26\\
    PN + Soft K-means\citep{ren2018metalearning}                  & 97.25 $\pm$ 0.10 & 50.09 $\pm$ 0.45 & 64.59 $\pm$ 0.28 & 51.52 $\pm$ 0.36 & 70.25 $\pm$ 0.31\\
    PN + Soft K-means + cluster\citep{ren2018metalearning}        & 97.68 $\pm$ 0.07 & 49.03 $\pm$ 0.24 & 63.08 $\pm$ 0.18 & 51.85 $\pm$ 0.25 & 69.42 $\pm$ 0.17\\
    PN + Masked soft K-means\citep{ren2018metalearning}           & 97.52 $\pm$ 0.07 & 50.41 $\pm$ 0.24 & 64.39 $\pm$ 0.24 &  52.39 $\pm$ 0.44 & 69.88 $\pm$ 0.20\\
    TPN-Semi~\citep{liu2018learning} &  N/A &  52.78 $\pm$ 0.27 & 66.42 $\pm$ 0.21 &  55.74 $\pm$ 0.29 &  71.01 $\pm$ 0.23\\
%    EGNN-Semi(T)~\citep{kim2019edge} &  N/A &  N/A & 64.32 & N/A & \textbf{80.15}\\
%    PRWN + Semi-supervised inference (Ours)              & \textbf{99.23} $\pm$ \textbf{0.08}   & \textbf{56.65} $\pm$ \textbf{0.24}  & \textbf{69.65} $\pm$ \textbf{0.20}\\
    PRWN + Semi-supervised inference (Ours) & \textbf{99.23} $\pm$ \textbf{0.08}   & \textbf{56.65} $\pm$ \textbf{0.24}  & \textbf{69.65} $\pm$ \textbf{0.20} & \textbf{59.17} $\pm$ \textbf{0.41}  & \textbf{71.06} $\pm$ \textbf{0.39}\\
    \end{tabular}
}
\end{table*}

    %  PN$_{all}$\citep{snell2017prototypical}  & 98.8                  & 49.4                  & 68.2 \\
    %  PN\citep{ren2018metalearning}    & 94.62 $\pm$ 0.09        & 43.61 $\pm$ 0.27        & 59.08 $\pm$ 0.22 \\
    %  \hline
    
    
    
    
    




